Cooperative Relative Localization in MAV Swarms with Ultra-wideband Ranging

Relative localization (RL) is essential for the successful operation of micro air vehicle (MAV) swarms. Achieving accurate 3-D RL in infrastructure-free and GPS-denied environments with only distance information is a challenging problem that has not been satisfactorily solved. In this work, based on the range-based peer-to-peer RL using the ultra-wideband (UWB) ranging technique, we develop a novel UWB-based cooperative relative localization (CRL) solution that integrates the relative motion dynamics of each host-neighbor pair to build a unified dynamic model and takes the distances between the neighbors as \textit{bonus information}. Observability analysis using differential geometry shows that the proposed CRL scheme can expand the observable subspace compared to other alternatives using only direct distances between the host agent and its neighbors. In addition, we apply the kernel-induced extended Kalman filter (EKF) to the CRL state estimation problem with the novel-designed Logarithmic-Versoria (LV) kernel to tackle heavy-tailed UWB noise. Sufficient conditions for the convergence of the fixed-point iteration involved in the estimation algorithm are also derived. Comparative Monte Carlo simulations demonstrate that the proposed CRL scheme combined with the LV-kernel EKF significantly improves the estimation accuracy owing to its robustness against both measurement outliers and incorrect measurement covariance matrix initialization. Moreover, with the LV kernel, the estimation is still satisfactory when performing the fixed-point iteration only once for reduced computational complexity.

==> acknowledgements.tex <==
\section*{Acknowledgments}
Acknowledgments

==> content_file/100.tex <==
\section{Modeling Framework}
\label{sec:3-prob}
In this section, we provide the modeling of the localization problem in detail. We will first present the relative motion dynamics between any pair of MAV agents. Next, we show the UWB noise modeling considering various practical issues (e.g., NLoS, multi-pathing, and transmission delay). Finally, the CRL modeling will be given based on the peer-to-peer dynamics and the noise model.

\subsection{Peer-to-peer Relative Motion Dynamics}
For a given MAV, the 3 axes of the body-fixed body frame ($\cF_{B}$) originate from the center of gravity of the robot with the $X$-axis pointing forward, $Z$-axis aligned to the direction of the thrust, and $Y$-axis completing the frame according to the right-handed convention. In addition, to simplify the localization problem, we mainly deal with the body-centered \textit{horizontal frame} ($\cF_{H}$) with its $Z$-axis being always \textit{perpendicular} to the ground plane \sven{\cite{li2020autonomous}}. With $\cF_{B}$ and $\cF_{H}$ defined, the orientation of both frames, as well as the transformation between the frames, can be determined using Euler angles (i.e., $\phi$, $\theta$, $\psi$) and the corresponding rotation matrices $\bR_X(\phi)$, $\bR_Y(\theta)$, and $\bR_Z(\psi)$.

In this work, the relative position is resolved in the horizontal frame $\cF_{H}$, and all related variables should be properly transformed accordingly. First, the velocity $\vv$ is measured in $\cF_{B}$ and it needs to be expressed in $\cF_{H}$. The rotation matrix transforming any vector in $\cF_{B}$ to $\cF_{H}$ is given as
\begin{equation}
    \label{eq:rotation_h2b}
    \hspace{-0.2cm}
    ^{H}\bR_{B} = \bR_Y(\theta)\bR_X(\phi) = 
    \begin{bmatrix}
    c(\theta) & s(\theta)s(\phi) & s(\theta)c(\phi) \\
    0 & c(\phi) & -s(\phi) \\
    -s(\theta) & c(\theta)s(\phi) & c(\theta)c(\phi)
    \end{bmatrix}.
\end{equation}
Second, the gyroscope measures the instantaneous angular velocity $\mathbf{\Omega}$ in $\cF_{B}$, to which the Euler angle rate should be properly related, and the formula is given as
\begin{equation}
    \label{eq:rotation_angular}
    \begin{bmatrix}
        \dot{\phi} \\
        \dot{\theta} \\
        \dot{\psi}
    \end{bmatrix}
    =
    \begin{bmatrix}
        1 & s(\phi)t(\theta) & c(\phi)t(\theta) \\
        0 & c(\phi) & -s(\phi) \\
        0 & s(\phi)/c(\theta) & c(\phi)/c(\theta)
    \end{bmatrix}
    \begin{bmatrix}
        {\Omega}_x \\
        {\Omega}_y \\
        {\Omega}_z
    \end{bmatrix}.
\end{equation}
In particular, we are interested in computing the heading rate $\dot{\psi}$, to which the changing of the horizontal frame is related. Note that the conversion in \eqref{eq:rotation_h2b} and \eqref{eq:rotation_angular} requires the roll ($\phi$) and pitch ($\theta$), both of which can be accurately estimated by IMU.

%\includegraphics[height=3cm]{example-image-a}
For any agent pair $(i,j)$, the peer-to-peer RL problem is defined as estimating the relative position of agent $j$ with respect to agent $i$ in agent $i$'s horizontal frame $\cF^i_{H}$. The state vector is thus given as $\x_{ij} = [\psi_{ij}, \p^\top_{ij}]$, where $\psi_{ij}$ is the relative heading and $\p_{ij} = [x_{ij}, y_{ij}, z_{ij}]^\top$ is the relative position in $\cF^i_{H}$. The control input of any agent $i$ is defined as $\uu_i = [\dot{\psi}_i, \vv^\top_i]^\top$ where $\vv_i = [v_{x,i}, v_{y,i}, v_{z,i}]^\top$ is the velocity input \sven{in $\cF^i_{H}$}, and the control input for agent pair $(i,j)$ is $\uu_{ij} = \vect\{\uu_i, \uu_j\}$. Then, the relative motion dynamics for agent pair $(i,j)$ can be derived using Newton's law as
\begin{equation}
    \label{eq:dy_pair}
    \dot{\x}_{ij} = \g(\x_{ij})\uu_{ij} = 
    \underbrace{
    \begin{bmatrix}
    \begin{array}{cc|cc}
        -1 & \mathbf{0}^\top_3 & 1 & \mathbf{0}^\top_3 \\
        -S\p_{ij} & -\mathds{I}_3 & \mathbf{0}_3 & \bR(\psi_{ij})
    \end{array}
    \end{bmatrix}}_{
    := 
    [\g^i(\x_{ij}) | \g^j(\x_{ij})]
    }
    \uu_{ij},
\end{equation}
and \eqref{eq:dy_pair} can be more compactly expressed as
\begin{equation}
    \label{eq:dy_pair_compact}
    \dot{\x}_{ij} = \g^c(\x_{ij}, \uu_{ij}) = 
    \begin{bmatrix}
        \dot{\psi}_j - \dot{\psi}_i \\
        \bR(\psi_{ij})\vv_j - \vv_i - S\dot{\psi}_i \p_{ij}
    \end{bmatrix}.
\end{equation}
In both \eqref{eq:dy_pair} and \eqref{eq:dy_pair_compact}, the matrices $\bR(\psi_{ij})$ and $S$ are given as
\begin{equation*}
    \bR(\psi_{ij}) = 
    \begin{bmatrix}
        c(\psi_{ij}) & -s(\psi_{ij}) & 0 \\
        s(\psi_{ij}) & c(\psi_{ij}) & 0 \\
        0 & 0 & 1 
    \end{bmatrix},
    \;
    S = 
    \begin{bmatrix}
        0 & -1 & 0 \\
        1 & 0 & 0 \\
        0 & 0 & 0
    \end{bmatrix}.
\end{equation*}
%\begin{remark}
    %The conversion equation in \eqref{eq:rotation_h2b} and \eqref{eq:rotation_angular} requires the roll ($\phi$) and pitch ($\theta$), both of which can be accurately estimated by IMU. Besides, integrating \eqref{eq:rotation_angular} can also be used to compute the 3 Euler angles.
%\end{remark}

\subsection{Heavy-tailed UWB Measurement Noise \& Delay Effects}
Ideally, the true distance $d^\ast_{ij}$ between agent pair $(i,j)$ is given in terms of its corresponding relative position $\p^\ast_{ij}$ as
\begin{equation}
    \label{eq:dis_model_ideal}
    d^\ast_{ij} = \| \p^\ast_{ij} \|.
\end{equation}
However, the measured distance deviates from the true value due to many practical factors. First, the distance measuring scheme in UWB is two-way ranging (TWR), whose noise model can be ideally assumed to be Gaussian considering only line-of-sight (LoS) scenarios. A more realistic noise model accounting for both multi-pathing and NLoS effects leads to a heavy-tailed distribution which is a linear combination of a Gaussian distribution and a Gamma distribution and other additional terms for outliers. We adopt the PDF of the simplified model \cite{pfeiffer2021computationally} for the noise $\nu$ as
\begin{equation}
    \label{eq:noise_pdf_sven}
    f(\nu) = \frac{1}{1+\sht}G(\nu; \sht \mu, \sigma) + \frac{\sht}{1+\sht}\gamma(\nu; k, \lambda),
\end{equation}
where \sven{$\sht \geq 0$} is a scale factor that \chang{is} chosen based on \chang{the} real measurement data.

Another source of measurement error comes from communication delay, especially for the indirect distance measurements between neighbors. Due to the limited bandwidth, the distances cannot be measured and transmitted simultaneously. Therefore, for agent $i$ which can only get the distance between its neighbors $j$ and $l$ through the communication between agent $j$ or $l$, the instantaneous true distance $\| \p^\ast_{jl} \|$ at the transmitting time $t_{\mathrm{tr}}$ differs from the transmitted $\| \p_{jl} \|$ measured at time $t_{\mathrm{ms}}$ due to the \chang{unknown} motion of agent $j$ and $l$ during the time interval $[t_{\mathrm{ms}}, t_{\mathrm{tr}}]$. Assume the length of the interval is upper bounded by $\bar{\eta}$, and the relative speed between any pair of agents is also bounded by $\bar{v}$, we have $\p^\ast_{jl} = \p_{jl} + \p_e = \p_{jl} + (\alpha\bar{\eta}\bar{v})\ii$ with $\alpha \in [0,1]$ and $\ii$ a \textit{unit} vector. For modeling simplicity, we further assume that $\ii$ has an equal probability of pointing in any direction and $\alpha$ is \textit{uniformly} distributed on $[0,1]$. Then, $\p_e$ has equal probability pointing at any point in a sphere \chang{of} radius $\bar{r} = \bar{\eta}\bar{v}$. As a result, the probability of having a distance error $\nu_d = s - d_{jl}$ is proportional to the area of the spherical cap of a sphere \chang{of} radius $s \in [d_{jl} - \bar{r}, d_{jl} + \bar{r}]$ intersected by a sphere with radius $\bar{r}$, and the area of the spherical cap can be \textit{approximated} as
\begin{equation}
    \label{eq:spherical_cap}
    a(\nu_d; d_{jl}, \bar{r}) = \pi[-(\nu_d^2 + 2\nu_dd_{jl}-\bar{r}^2)^2 + 4d_{jl}^2\bar{r}^2 ].
\end{equation}
Following \eqref{eq:spherical_cap}, the normalized PDF of $\nu_d$ is thus given as
\begin{equation}
    \label{eq:noise_pdf_changrui}
    \hspace{-0.35cm}
    f(\nu_d) = \frac{15}{16 \pi \bar{r}^3(5d^2_{jl} - \bar{r}^2)} a(\nu_d; d_{jl}, \bar{r}),\; (\nu_d \in [-\bar{r}, \bar{r}]).
\end{equation}
\sven{The severity of the delay effects hinges on the velocity of the MAV and the density of the swarm. On the one hand, if the MAVs are flying at high speed, then $\bar{v}$ can be large. On the other hand, if the swarm is too dense such that the number of neighbors of each agent is big, then $\bar{\eta}$ can be quite large due to limited bandwidth. In Fig. \ref{fig:delaynoise}, we present some representative PDFs when $\bar{r} = 0.15\munit$.}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/delaynoise.pdf}
    \caption{PDFs of noise $\nu_d$}
    \label{fig:delaynoise}
\end{figure}
%\includegraphics[height=2cm]{example-image-b}
\begin{remark}
    The noise $\nu$ and $\nu_d$ are independent, which explains why they are considered separately instead of being combined into a single type of noise with a unified PDF.
\end{remark}
\begin{remark}
    The approximation in \eqref{eq:spherical_cap} is valid under the condition that $\bar{r} \ll d_{jl}$. This condition holds in general given that two MAVs do not fly in a dangerous mode within a pretty short distance range and the number of neighbors for any agent is limited such that $\bar{\eta}$ does not permit a large value.
\end{remark}

\subsection{Modeling of CRL Schemes} 
Having the peer-to-peer relative motion dynamics established as in \eqref{eq:dy_pair}, we then move forward to the CRL modeling. Consider a swarm of $N$ agent, and for agent $i$, the set of its neighbors is $\mathcal{N}_{i}$ with $|\mathcal{N}_{i}| = N_{i}$. We explicitly express $\mathcal{N}_{i}$ as $\{j_{\alpha} \in \mathbb{Z}^+_{N}|j_{\alpha} \neq i, j_{\alpha} < j_{\alpha+1}\;(\alpha = 1,2,\cdots,N_{i})\}$.%Without loss of generality, we can always tale $i = 1$, then $\mathcal{N}_{i}$ becomes $\mathbb{Z}^2_{N}$.
To build an integrated dynamic model, we augment the state $\x_{ij_\alpha}$ of agent pair $(i,j_\alpha)$, and the augmented state $\bar{\x}_i$ is given as
\begin{equation*}
    \label{eq:aug_state}
    \bar{\x}_i = \textstyle\vect^{N_i}_{\alpha=1}\{\x_{ij_\alpha}\}.
\end{equation*}
We also augment the control input $\uu_i$ to form $\bar{\uu}$ as
\begin{equation*}
    \label{eq:aug_control}
    \bar{\uu}_i = \vect\{\uu_i, \textstyle\vect^{N_i}_{\alpha=1} \{\uu_{j_\alpha}\} \}.
\end{equation*}
To construct the control coupling matrix $\bar{\g}_i(\bar{\x}_i)$ for $\bar{\uu}_i$, we first define auxiliary matrix $\g_a(\x_{ij_\alpha})$ for all $j_\alpha \in \mathcal{N}_{i}$ as
\begin{equation}
    \label{eq:aug_control_matrix_aux}
    \g_a(\x_{ij_\alpha}) \lsdeng \bb^{N_i+1}_1 \otimes \g^i(\x_{ij_\alpha}) + \bb^{N_i+1}_{\alpha+1} \otimes \g^{j_\alpha}(\x_{ij_\alpha}),
\end{equation}
where $\g^i(\x_{ij_\alpha})$ and $\g^{j_\alpha}(\x_{ij_\alpha})$ are defined in \eqref{eq:dy_pair}. Correspondingly, $\bar{\g}_i(\bar{\x}_i)$ can be built as
\begin{equation}
    \label{eq:aug_control_matrix}
    \bar{\g}_i(\bar{\x}_i) = \textstyle\vect^{N_i}_{\alpha=1}\{\g_a(\x_{ij_\alpha})\}.
\end{equation}
Finally, the integrated motion dynamics in terms of state $\bar{\x}_i$ driven by control $\bar{\uu}$ is given as
\begin{equation}
    \label{eq:dy_aug}
    \dot{\bar{\x}}_i = \bar{\g}_i(\bar{\x}_i)\bar{\uu}_i.
\end{equation}
Following \eqref{eq:dy_pair_compact}, we can also define $\bar{\g}^c_i(\bar{\x}_i, \bar{\uu})$ similarly as
\begin{equation}
    \label{eq:aug_control_matrix_compact}
    \bar{\g}^c_i(\bar{\x}_i, \bar{\uu}_i) = \textstyle\vect^{N_i}_{\alpha=1}\{\g^c(\x_{ij_\alpha}, \uu_{ij_\alpha})\} ,
\end{equation}
and a compact form directly follows as
\begin{equation}
    \label{eq:dy_aug_compact}
    \dot{\bar{\x}}_i = \bar{\g}^c_i(\bar{\x}_i, \bar{\uu}_i).
\end{equation}

For the measurement model of CRL, we first augment the direct distance model between agent $i$ and each of its neighbors
\begin{equation}
    \label{eq:dis_direct}
    \hh^\mathrm{d}_i(\bar{\x}_i) = \textstyle\vect^{N_i}_{\alpha=1}\{\|\p_{ij_\alpha}\|\}.
\end{equation}
Then, the augmented direct measurement considering only the noise $\nu$ is given as
\begin{equation}
    \label{eq:dis_direct_noisy}
    \y^\mathrm{d}_i = \hh^\mathrm{d}_i(\bar{\x}_i) + \bm{\nu},
\end{equation}
where $\bm{\nu} = \textstyle\diag^{N_i}_{\alpha=1}\{\nu_\alpha\}$ is the augmented noise. On the other hand, the augmented indirect distances transmitted by agent $j_\alpha$ are given as
\begin{equation}
    \label{eq:dis_indirect_neighborwise}
    \hh^\mathrm{id}_i(\bar{\x}_i; j_\alpha) = \textstyle\vect_{\{l \in \mathcal{N}_{i} \cap \mathcal{N}_{j_\alpha} \}}\{ \|\p_{ij_\alpha} - \p_{il}\| \},
\end{equation}
and the augmented indirect distances considering all its neighbors follows as
\begin{equation}
    \label{eq:dis_indirect_all}
    \hh^\mathrm{id}_i(\bar{\x}_i) = \textstyle\vect^{N_i}_{\alpha = 1}\{ \hh^\mathrm{id}_i(\bar{\x}_i; j_\alpha)\}.
\end{equation}
The final noisy indirect measurement model is given as
\begin{equation}
    \label{eq:dis_indirect_noisy}
    \y^\mathrm{id}_i = \hh^\mathrm{id}_i(\bar{\x}_i) + \bm{\nu}_a
\end{equation}
where $\bm{\nu}_a = \textstyle\diag^{p_{\mathrm{id}}}_{\beta=1}\{\nu_\beta + \nu_{d,\beta}\}$ with $p_{\mathrm{id}} = \sum^{N_i}_{\alpha=1}|\mathcal{N}_{i} \cap \mathcal{N}_{j_\alpha}|$.

Moreover, we assume that all velocity inputs are imperfect due to actuator noise $\Delta \uu_i$ for agent $i$, with which we also define $\Delta \uu_{ij_\alpha} = \vect\{\Delta \uu_i, \Delta \uu_{j_\alpha}\}$ and $\Delta \bar{\uu}_i = \vect\{\Delta \uu_i, \textstyle\vect^{N_i}_{\alpha=1} \{\Delta \uu_{j_\alpha}\} \}$. Referring to \eqref{eq:dy_aug}, \eqref{eq:dis_direct_noisy} and \eqref{eq:dis_indirect_noisy}, the full-CRL (fCRL) model with the augmented dynamics and both direct and indirect measurements is given as
\begin{equation}
\label{eq:fcrl}
    \text{fCRL}:\left \{
    \begin{aligned}
    \dot{\bar{\x}}_i &= \bar{\g}_i(\bar{\x}_i)(\bar{\uu}_i + \Delta\bar{\uu}_i) \\
    \begin{bmatrix}
        \y^\mathrm{d}_i \\
        \y^\mathrm{id}_i
    \end{bmatrix}
    &=
    \begin{bmatrix}
        \hh^\mathrm{d}_i(\bar{\x}_i) \\
        \hh^\mathrm{id}_i(\bar{\x}_i)
    \end{bmatrix}
    +
    \begin{bmatrix}
        \bm{\nu} \\
        \bm{\nu}_a
    \end{bmatrix}
    \end{aligned}
    \right. .
\end{equation}

For comparative study, we also introduce the following two models: i) the half-CRL (hCRL) model with the augmented dynamics and only direct measurements, ii) the non-CRL (nCRL) model which is simply \textit{a collection} of the peer-to-peer dynamics in \eqref{eq:dy_pair} for agent pairs $(i,j_\alpha)$ without state and input augmentation, \sven{$\forall j_\alpha \in \mathcal{N}_i$}. The details are given below:
% hCRL modeling
\begin{equation}
\label{eq:hcrl}
    \hspace{-3.3cm}
    \text{hCRL}:\left \{
    \begin{aligned}
    \dot{\bar{\x}}_i &= \bar{\g}_i(\bar{\x}_i)(\bar{\uu}_i + \Delta\bar{\uu}_i) \\
        \y^\mathrm{d}_i
    &=
        \hh^\mathrm{d}_i(\bar{\x}_i)
    +
        \bm{\nu} 
    \end{aligned}
    \right. ,
\end{equation}
% nCRL modeling
\begin{equation}
\label{eq:ncrl}
    %\hspace{0cm}
    \text{nCRL}:\bigg\{ \left \{
    \begin{aligned}
    \dot{\x}_{ij_\alpha} &= \g(\x_{ij_\alpha})(\uu_{ij_\alpha} + \Delta \uu_{ij_\alpha})\\
    y_{ij_\alpha} &= \|\p_{ij_\alpha}\| + \nu_\alpha
    \end{aligned}
    \right. \bigg\}_{\{j_\alpha \in \mathcal{N}_i\}}.
\end{equation}
\begin{remark}
    The 3 dynamic models (i.e., fCRL, hCRL, and nCRL) are all continuous-time nonlinear control systems. In addition, they are all \textit{drift-free} and \textit{input-affine}, which perfectly fits the general system description in \eqref{eq:sys_math}.
\end{remark}
\begin{remark}
    Due to actuator and measurement noise, the built models are \textit{stochastic} in nature. Thus, applying nonlinear filtering techniques is necessary for state estimation.
\end{remark}



==> content_file/102.tex <==
\section{Preliminaries}
\label{sec:2-pre}
\subsection{Notation and Definitions}
\vspace{-0.05cm}
Let $x \in \R^n$ denote a vector with $x[k]$ and $\| {x} \|_p (p \in \{1,2,\infty\})$ being its $k$-th element and vector $p$-norm. $M\in\R^{n\times m}$ is a matrix with $M^\top$, $M[k]$ and $M^\top[k]$ being its transpose, $k$-th row and $k$-th column, respectively. Similarly, $\| {M} \|_p (p \in \{1,2,\infty\})$ denotes the induced matrix $p$-norm. In the sequel, all norms will be referred to as $2$-norm if not explicitly specified. The set of positive integers up to $n$ %and the set of non-negative integers up to $n$ 
is $\mathbb{Z}_n^{+}$, and $\mathbb{Z}_{j}^{i}$ denotes non-negative integers from $i$ to $j \; (0\leq i\leq j)$. 

The minimum (maximum) eigenvalue of a matrix $M$ is denoted as $\lambda_{\text{min}}(M)$ ($\lambda_{\text{max}}(M)$). Given $x, y \in \R^n$, $x/y$ means element-wise division. \sven{$\otimes$ is the Kronecker product used for matrices (vectors).} $\mathbf{0}_n$, $\mathds{1}_n$, and $\mathds{I}_n$ are $n$-dimensional zero vector, one vector, and identity matrix, respectively. The $n$-dimensional basis row vector with the $i$-th entry being 1 while all other entries being 0 is denoted as $\bb^n_i$. Further, we define operators $\diag$ and $\vect$ for matrices (vectors) as: % are defined as follows:
%\vspace{0.1cm}
\begin{align*}
    \begin{aligned}
    \small
    %&\hspace{-0.1cm}\textstyle\diag_N \{ M_i\} = \mathds{I}_N \otimes M_i \; ,  
	%&\hspace{-0.3cm}  \textstyle\vect_N \{M_i\} = \mathds{1}_N \otimes M_i \; ,\\[-0.1cm]
    %&\hspace{-0.1cm}\textstyle\diag_N \{ M_i\} = \mathds{I}_N \otimes M_i \; ,  
	%&\hspace{-0.3cm}  \textstyle\vect_N \{M_i\} = \mathds{1}_N \otimes M_i \; ,\\
	%\end{aligned}
	%\begin{aligned}
	&\hspace{-0.1cm} \textstyle\diag \{ M_i, M_j\} = \begin{bmatrix} M_i & \mathbf{0} \\  \mathbf{0} & M_j \end{bmatrix},
    &\hspace{-0.2cm} \textstyle\vect \{ M_i, M_j\} = \begin{bmatrix} M_i  \\ M_j \end{bmatrix}, 
        \end{aligned}
\end{align*}
\begin{align*}
    \begin{aligned}
    \small
    &\hspace{-0.1cm} \textstyle\diag_{k=i}^j \{ M_k\} = \begin{bmatrix} M_i & &\\[-0.1cm] & \ddots & \\[-0.1cm] & & M_j \end{bmatrix}, \;
    &\hspace{-0.2cm} \textstyle\vect_{k=i}^j \{ M_k\} = \begin{bmatrix} M_i \\[-0.1cm] \vdots \\[-0.1cm] M_j \end{bmatrix},
    \end{aligned}
\end{align*}
and for $\textstyle\diag_{k=i}^j \{ \cdot \} $ and $\textstyle\vect_{k=i}^j \{ \cdot \}$, in case $j<i$, the operators produce \textit{no outcome} and can be ignored whenever occurs.

For convenience, the trigonometric functions $\sin(\cdot)$, $\cos(\cdot)$ and $\tan(\cdot)$ are abbreviated as $s(\cdot)$, $c(\cdot)$ and $t(\cdot)$, respectively. The Cholesky decomposition for matrices is denoted as a function $\mathcal{C}\mathcal{H}(\cdot)$. Besides, the probability density function (PDF) of a random variable $X$ obeying Gaussian distribution is denoted as $G(x; m,\sigma)$ with $m$ being the mean and $\sigma$ being the standard deviation. For Gamma distribution, we use $\gamma(x; k,\lambda) = [\Gamma(k)]^{-1}\lambda^kx^{k-1}\mathrm{exp}(-\lambda x)$, where $\Gamma(\cdot)$ is the gamma function. Lastly, the uniform distribution on interval $[a, b]$ is denoted as $U(a,b)$.

\subsection{Kernel Induced Correntropy}
In information theoretical learning, correntropy measures the similarity between two random variables $X, Y \in \mathbb{R}$ as
\begin{equation}
    \label{eq:corr_definition}
    C(X,Y) = \mathbb{E}[\kappa(X,Y)] = \int \kappa(x,y)\mathrm{d}F_{XY}(x,y),
\end{equation}
where $F_{XY}(x,y)$ is the joint distribution function and $\kappa(\cdot,\cdot)$ is a shift-invariant Mercer kernel. In this work, inspired by the Versoria function, we design a novel Logarithmic-Versoria (LV) kernel as
\begin{equation}
    \label{eq:ker_definition}
    \kappa(x,y) = V_{\tau}(e) = \frac{\tau}{\tau + \ln(1 + e^2)},
\end{equation}
where $e=x-y$ is the error, and $\tau > 0$ controls the \textit{bandwidth} of the kernel. The Versoria function can exploit the non-Gaussian characteristics and provide better higher-order error information than the Gaussian kernel \cite{huang2017maximum}. The newly designed LV kernel not only inherits the power of Versoria function but also exhibits smoother behavior for small errors. A brief comparison of different kernel functions is given in Figure \ref{fig:kernel}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/kernelplot.pdf}
    \caption{Kernel Function Comparison}
    \label{fig:kernel}
\end{figure}

For the filtering problem of general stochastic systems where the analytical distribution of the state(output) is not attainable, it is practical to approximate the correntropy using the sampled-mean strategy as
\begin{equation}
    \label{eq:corr_sample}
    \hat{C}(X,Y) = \frac{1}{L}\sum^{L}_{i=1}V_{\tau}(e(i)),
\end{equation}
where $e(i)=x(i)-y(i)$ with $\{x(i),y(i)\}$ being the candidate data points. Following the sampled-mean correntropy, a generalized measure is using multi-kernel with varying bandwidth (i.e., $V_{\tau_i}(e(i))$ in \eqref{eq:corr_sample}), which enables more design flexibility and can scale the measure for different candidates.

\subsection{Knowledge from Differential Geometry}
Consider a drift-free input-affine nonlinear control system
\begin{equation}
\label{eq:sys_math}
\left \{
\begin{aligned}
    \dot{\x} &= \sum\nolimits^{m}_{i=1}\g_{i}(\x,t)u_i \\
    \y &= [h_1(\x), h_2(\x), \cdots, h_p(\x)]^\top
\end{aligned}
\right. ,
\end{equation}
where $\x$ evolves in a $\mathcal{C}^\infty-\text{manifold}$ $\mathcal{M}$ of dimension $n$, $\g_{i}(\x,t)$ are time-varying (TV) vector fields in $\mathcal{M}$, and $h_i(\x)$ are time-invariant (TI) scalar fields also defined on $\mathcal{M}$. Besides, all functions are $\mathcal{C}^\infty$ functions of their arguments. The time $t$ belongs to an open interval $\mathcal{I}\subseteq \mathbb{R}$, and we denote $\uM = \mathcal{I}\times \mathcal{M}$. To analyze the above system, we present some basic differential geometric tools.
\begin{definition}[Lie Derivative]
Given a scalar function $h(\x):\mathcal{M} \mapsto \mathbb{R}$, and a vector field $\g(\x,t): \uM \mapsto \mathcal{M}$. The \textit{Lie derivative} of a covector $\mathrm{d}h$ with respect to $\x$ is defined as
\begin{equation}
    \label{eq:lie_derivative}
    \cL_{\g}\mathrm{d}h = \mathrm{d}(\cL_{\g}h) = \mathrm{d}(\langle \frac{\partial h}{\partial \x}, \g(\x,t)\rangle),
\end{equation}
where $\mathrm{d}h$, being the dual of $\g(\x,t)$, is a special type of covector called \textit{exact differential}, \sven{and $\langle \cdot,\cdot\rangle$ denotes the inner product of two vector fields}. Further, a set of \textit{covectors} $\mathrm{d} h_i$ can form a \textit{codistribution} $\Xi = \text{span}\{\mathrm{d} h_i\}$\cite{isidori1985nonlinear}, and the Lie derivative of the codistribution is $\cL_{\g}\Xi = \text{span}\{\cL_{\g}\xi | \forall \xi \in \Xi\}$. 
%In addition, the Lie derivative can be recursively defined as
%\begin{equation}
%\label{eq:lie_recursion}
    %\cL^r_{\g}\mathrm{d}h = \mathrm{d}(\cL^r_{\g}h) = \mathrm{d}(\langle \cL^{r-1}_{\g}\mathrm{d}h, \g \rangle) \;(r \geq 1), 
%\end{equation}
\end{definition}
%with the special case being $\cL^0_{\g}\mathrm{d}h := \mathrm{d}h$.

To analyze the time-varying system in \eqref{eq:sys_math}, we introduce the \textit{augmented Lie derivative} \cite{martinelli2022extension} for a covector $\mathrm{d}h$ as
\begin{equation}
    \label{eq:lie_newoperator}
    \dot{\cL}_{\g}\mathrm{d}h = \cL_{\g}\mathrm{d}h + \frac{\partial \mathrm{d}h}{\partial t}.
\end{equation}
Besides, this new derivative permits a recursive operation as
\begin{equation}
    \dot{\cL}^r_{\g}\mathrm{d}h = \dot{\cL}_{\g}(\dot{\cL}^{r-1}_{\g}\mathrm{d}h),  \quad (r \in \mathbb{Z}_+),
\end{equation}
with the initial case being $\dot{\cL}^0_{\g}\mathrm{d}h := \mathrm{d}h$. Likewise, the augmented Lie derivative can also act upon codistributions. The above geometric tools will be used for the \textit{observability} analysis in Section \ref{sec:4-mainapp}.

==> content_file/103.tex <==
\subsection{Filtering Settings}
In the simulation, the filter run at the discrete time $k\Delta t$ with the sampling interval $\Delta t = 0.01 \tunit$. When doing state estimation, the filter receives the body velocities and heading rate derived from the nominal input for prediction and then uses the noisy distance measurements for state correction. In the following, we will elaborate on the initialization settings and the noise covariance settings of the filter.

First, the filter does not know the true initial state (i.e., the true relative position and relative heading). Given the true initial \textit{global} state tuple $\{\psi_0, x_c\lsjia R\cos(\varphi), y_c\lsjia R\sin(\varphi), z_c\}$ of all the $5$ agents, the true initial state $\x_{ij}(0)$ for any pair $(i,j)$ can be computed, based on which the true state $\x_i(0)$ for the CRL task of agent $i$ can be built by state augmentation. Then, we manually add initial offset $\Delta \x_{ij}(0) = [\Delta \psi_0, \Delta x_0, \Delta y_0, \Delta z_0]^\top$ to the initial state, where the heading uncertainty is simply $\psi_0 \sim U(-\bar{\psi}_e, \bar{\psi}_e)$ and the position uncertainty is designed as 
\begin{equation}
    \label{eq:position uncertainty}
    \left \{
    \begin{aligned}
        \Delta x_0 &= \bar{r}_e \cos(\varrho)\cos(\varphi) \\
        \Delta y_0 &= \bar{r}_e \cos(\varrho) \sin(\varphi) \\
        \Delta z_0 &= \bar{r}_e \sin(\varrho)
    \end{aligned}
    \right. ,
\end{equation}
where $\varrho \sim U(-\pi/2, \pi/2)$ and $\varphi \sim U(0, 2\pi)$. In other words, the design rule in \eqref{eq:position uncertainty} ensures that the initial position error has a fixed length $\bar{r}_e$ whereas its direction is unknown. Following the state augmentation modeling in Section \ref{sec:4-mainapp}, for an agent $i$ and its neighbors $\mathcal{N}_i$, we first build $\Delta \x_i(0) = \textstyle\vect^{N_i}_{\alpha=1}\{\Delta \x_{ij_\alpha}(0)\}$ where $\Delta \x_{ij_\alpha}(0)$ are repeatedly generated using the same \textit{uncertainty level} pair $(\bar{\psi}_e, \bar{r}_e)$, then the initial state of the filter is given by $\hat{\x}^+(0) = \x_i(0) + \Delta \x_i(0)$. Correspondingly, the initial covariance is set as $\bP^+(0) = \mathds{I}_{N_i} \otimes \bP_e$, where $\bP_e = \diag\{\bar{\psi}_e^2/3, \bar{r}_e^2/4, \bar{r}_e^2/4, \bar{r}_e^2/2\}$. 

Apart from the initialization, the filters should have some prior knowledge of the noise. We assume that the filter has access to the true actuator covariance matrix $\mathbf{Q}_{\uu}$. For nCRL scheme where pairwise localization is the foundation, we set $\Q_k = \diag\{\Q_{\uu}, \Q_{\uu}\}$ (cf. step 22 of Algorithm \ref{algorithm2}), whereas for fCRL and hCRL schemes, we have $\Q_k = \mathds{I}_{N_i+1} \otimes \Q_{\uu}$ (cf. step 14 of Algorithm \ref{algorithm2}). As for the measurement covariance matrix, we have the following two modes: 
\begin{itemize}
    \item \textbf{Smart}: The filter knows the heavy-tailed outliers and also the time delay.
    \item \textbf{Inattentive}: The filter is unaware of the heavy-tailed outliers or the time delay and assumes the UWB noise to be Gaussian distributed (i.e., $\sht = 0$ in \eqref{eq:noise_pdf_sven}).
\end{itemize}
Based on the noise parameters in Table \ref{tb:noise_parameters}, we can numerically obtain $\sigma^2_{\nu} \approx 0.08$ and $\sigma^2_{\nu_d} \approx 0.01$. The details of the measurement covariance matrix $\mathbf{R}_k$ for both of the settings are summarized in Table \ref{tb:meas_noise_variance}.
\begin{table}[htbp]
\renewcommand\arraystretch{1.2}\small
  \centering
  \caption{Measurement Covariance Matrix $\mathbf{R}_k$}
  \label{tb:meas_noise_variance}
  \begin{tabular}{c|c|c}
    \toprule
    % Formulation & TAMD & MI \\
         & Smart & Inattentive \\
    \midrule
    \midrule
        fCRL & $\diag\{0.08\mathds{I}_{N_i}, 0.09\mathds{I}_{p_{\text{id}}}\}$ & $0.01\mathds{I}_{(N_i+p_{\text{id}})}$ \\
        hCRL & $0.08\mathds{I}_{N_i}$ & $0.01\mathds{I}_{N_i}$ \\
        nCRL & $0.08$ & $0.01$ \\
    \bottomrule
 \end{tabular}
\end{table}

==> content_file/2.2-p2p-dynamics.tex <==
\subsection{Peer-to-peer Relative Motion Dynamics}
\chang{We first introduce the relative motion dynamics for a pair of agents, which is the basic building block of the CRL models in later stages.} For a given MAV, the 3 axes of the body-fixed body frame ($\cF_{B}$) originate from the center of gravity of the robot with the $X$-axis pointing forward, $Z$-axis \chang{being} aligned to the direction of the thrust, and $Y$-axis completing the frame according to the right-handed convention. In addition, to simplify the localization problem, we mainly deal with the body-centered \textit{horizontal frame} ($\cF_{H}$) with its $Z$-axis being always \textit{perpendicular} to the ground plane \sven{\cite{li2020autonomous}}. With $\cF_{B}$ and $\cF_{H}$ defined, the orientation of both frames, as well as the transformation between the frames, can be determined using Euler angles (i.e., $\phi$, $\theta$, $\psi$) and the corresponding rotation matrices $\bR_X(\phi)$, $\bR_Y(\theta)$, and $\bR_Z(\psi)$.

In this work, the relative position is resolved in the horizontal frame $\cF_{H}$, and all related variables should be properly transformed accordingly. First, the velocity $\vv$ is measured in $\cF_{B}$ and it needs to be expressed in $\cF_{H}$. The rotation matrix transforming any vector in $\cF_{B}$ to $\cF_{H}$ is given as
\begin{equation}
    \label{eq:rotation_h2b}
    \hspace{-0.2cm}
    ^{H}\bR_{B} = \bR_Y(\theta)\bR_X(\phi) = 
    \begin{bmatrix}
    c(\theta) & s(\theta)s(\phi) & s(\theta)c(\phi) \\
    0 & c(\phi) & -s(\phi) \\
    -s(\theta) & c(\theta)s(\phi) & c(\theta)c(\phi)
    \end{bmatrix}.
\end{equation}
Second, the gyroscope measures the instantaneous angular velocity $\mathbf{\Omega}$ in $\cF_{B}$, to which the Euler angle rate should be properly related, and the formula is given as
\begin{equation}
    \label{eq:rotation_angular}
    \begin{bmatrix}
        \dot{\phi} \\
        \dot{\theta} \\
        \dot{\psi}
    \end{bmatrix}
    =
    \begin{bmatrix}
        1 & s(\phi)t(\theta) & c(\phi)t(\theta) \\
        0 & c(\phi) & -s(\phi) \\
        0 & s(\phi)/c(\theta) & c(\phi)/c(\theta)
    \end{bmatrix}
    \begin{bmatrix}
        {\Omega}_x \\
        {\Omega}_y \\
        {\Omega}_z
    \end{bmatrix}.
\end{equation}
In particular, we are interested in computing the heading rate $\dot{\psi}$, to which the changing of the horizontal frame is related. Note that the conversion in \eqref{eq:rotation_h2b} and \eqref{eq:rotation_angular} requires the roll ($\phi$) and pitch ($\theta$), both of which can be accurately estimated by IMU.

%\includegraphics[height=3cm]{example-image-a}
For any agent pair $(i,j)$, the peer-to-peer RL problem is defined as estimating the relative position of agent $j$ with respect to agent $i$ in agent $i$'s horizontal frame $\cF^i_{H}$. The state vector is thus given as $\x_{ij} = [\psi_{ij}, \p^\top_{ij}]$, where $\psi_{ij}$ is the relative heading and $\p_{ij} = [x_{ij}, y_{ij}, z_{ij}]^\top$ is the relative position in $\cF^i_{H}$. The control input of any agent $i$ is defined as $\uu_i = [\dot{\psi}_i, \vv^\top_i]^\top$ where $\vv_i = [v_{x,i}, v_{y,i}, v_{z,i}]^\top$ is the velocity input \sven{in $\cF^i_{H}$}, and the control input for agent pair $(i,j)$ is $\uu_{ij} = \vect\{\uu_i, \uu_j\}$. Then, the relative motion dynamics for agent pair $(i,j)$ can be derived using Newton's law as
\begin{equation}
    \label{eq:dy_pair}
    \dot{\x}_{ij} = \g(\x_{ij})\uu_{ij} = 
    \underbrace{
    \begin{bmatrix}
    \begin{array}{cc|cc}
        -1 & \mathbf{0}^\top_3 & 1 & \mathbf{0}^\top_3 \\
        -S\p_{ij} & -\mathds{I}_3 & \mathbf{0}_3 & \bR(\psi_{ij})
    \end{array}
    \end{bmatrix}}_{
    := 
    [\g^i(\x_{ij}) | \g^j(\x_{ij})]
    }
    \uu_{ij},
\end{equation}
and \eqref{eq:dy_pair} can be more compactly expressed as
\begin{equation}
    \label{eq:dy_pair_compact}
    \dot{\x}_{ij} = \g^c(\x_{ij}, \uu_{ij}) = 
    \begin{bmatrix}
        \dot{\psi}_j - \dot{\psi}_i \\
        \bR(\psi_{ij})\vv_j - \vv_i - S\dot{\psi}_i \p_{ij}
    \end{bmatrix}.
\end{equation}
In both \eqref{eq:dy_pair} and \eqref{eq:dy_pair_compact}, the matrices $\bR(\psi_{ij})$ and $S$ are given as
\begin{equation*}
    \bR(\psi_{ij}) = 
    \begin{bmatrix}
        c(\psi_{ij}) & -s(\psi_{ij}) & 0 \\
        s(\psi_{ij}) & c(\psi_{ij}) & 0 \\
        0 & 0 & 1 
    \end{bmatrix},
    \;
    S = 
    \begin{bmatrix}
        0 & -1 & 0 \\
        1 & 0 & 0 \\
        0 & 0 & 0
    \end{bmatrix}.
\end{equation*}
%\begin{remark}
    %The conversion equation in \eqref{eq:rotation_h2b} and \eqref{eq:rotation_angular} requires the roll ($\phi$) and pitch ($\theta$), both of which can be accurately estimated by IMU. Besides, integrating \eqref{eq:rotation_angular} can also be used to compute the 3 Euler angles.
%\end{remark}

==> content_file/3.1-ThreeCRL-Models.tex <==
\subsection{Modeling of CRL Schemes} 
Having the peer-to-peer relative motion dynamics established as in \eqref{eq:dy_pair}, we then move forward to the CRL modeling. Consider a swarm of $N$ agent, and for agent $i$, the set of its neighbors is $\mathcal{N}_{i}$ with $|\mathcal{N}_{i}| = N_{i}$. We explicitly express $\mathcal{N}_{i}$ as $\{j_{\alpha} \in \mathbb{Z}^+_{N}|j_{\alpha} \neq i, j_{\alpha} < j_{\alpha+1}\;(\alpha = 1,2,\cdots,N_{i})\}$.%Without loss of generality, we can always tale $i = 1$, then $\mathcal{N}_{i}$ becomes $\mathbb{Z}^2_{N}$.
To build an integrated dynamic model, we augment the state $\x_{ij_\alpha}$ of agent pair $(i,j_\alpha)$, and the augmented state $\bar{\x}_i$ is given as
\begin{equation*}
    \label{eq:aug_state}
    \bar{\x}_i = \textstyle\vect^{N_i}_{\alpha=1}\{\x_{ij_\alpha}\}.
\end{equation*}
We also augment the control input $\uu_i$ to form $\bar{\uu}$ as
\begin{equation*}
    \label{eq:aug_control}
    \bar{\uu}_i = \vect\{\uu_i, \textstyle\vect^{N_i}_{\alpha=1} \{\uu_{j_\alpha}\} \}.
\end{equation*}
To construct the control coupling matrix $\bar{\g}_i(\bar{\x}_i)$ for $\bar{\uu}_i$, we first define auxiliary matrix $\g_a(\x_{ij_\alpha})$ for all $j_\alpha \in \mathcal{N}_{i}$ as
\begin{equation}
    \label{eq:aug_control_matrix_aux}
    \g_a(\x_{ij_\alpha}) \lsdeng \bb^{N_i+1}_1 \otimes \g^i(\x_{ij_\alpha}) + \bb^{N_i+1}_{\alpha+1} \otimes \g^{j_\alpha}(\x_{ij_\alpha}),
\end{equation}
where $\g^i(\x_{ij_\alpha})$ and $\g^{j_\alpha}(\x_{ij_\alpha})$ are defined in \eqref{eq:dy_pair}. Correspondingly, $\bar{\g}_i(\bar{\x}_i)$ can be built as
\begin{equation}
    \label{eq:aug_control_matrix}
    \bar{\g}_i(\bar{\x}_i) = \textstyle\vect^{N_i}_{\alpha=1}\{\g_a(\x_{ij_\alpha})\}.
\end{equation}
Finally, the integrated motion dynamics in terms of state $\bar{\x}_i$ driven by control $\bar{\uu}$ is given as
\begin{equation}
    \label{eq:dy_aug}
    \dot{\bar{\x}}_i = \bar{\g}_i(\bar{\x}_i)\bar{\uu}_i.
\end{equation}
Following \eqref{eq:dy_pair_compact}, we can also define $\bar{\g}^c_i(\bar{\x}_i, \bar{\uu})$ similarly as
\begin{equation}
    \label{eq:aug_control_matrix_compact}
    \bar{\g}^c_i(\bar{\x}_i, \bar{\uu}_i) = \textstyle\vect^{N_i}_{\alpha=1}\{\g^c(\x_{ij_\alpha}, \uu_{ij_\alpha})\} ,
\end{equation}
and a compact form directly follows as
\begin{equation}
    \label{eq:dy_aug_compact}
    \dot{\bar{\x}}_i = \bar{\g}^c_i(\bar{\x}_i, \bar{\uu}_i).
\end{equation}

For the measurement model of CRL, we first augment the direct distance model between agent $i$ and each of its neighbors
\begin{equation}
    \label{eq:dis_direct}
    \hh^\mathrm{d}_i(\bar{\x}_i) = \textstyle\vect^{N_i}_{\alpha=1}\{\|\p_{ij_\alpha}\|\}.
\end{equation}
Then, the augmented direct measurement considering only the noise $\nu$ is given as
\begin{equation}
    \label{eq:dis_direct_noisy}
    \y^\mathrm{d}_i = \hh^\mathrm{d}_i(\bar{\x}_i) + \bm{\nu},
\end{equation}
where $\bm{\nu} = \textstyle\diag^{N_i}_{\alpha=1}\{\nu_\alpha\}$ is the augmented noise. On the other hand, the augmented indirect distances transmitted by agent $j_\alpha$ are given as
\begin{equation}
    \label{eq:dis_indirect_neighborwise}
    \hh^\mathrm{id}_i(\bar{\x}_i; j_\alpha) = \textstyle\vect_{\{l \in \mathcal{N}_{i} \cap \mathcal{N}_{j_\alpha} \}}\{ \|\p_{ij_\alpha} - \p_{il}\| \},
\end{equation}
and the augmented indirect distances considering all its neighbors follows as
\begin{equation}
    \label{eq:dis_indirect_all}
    \hh^\mathrm{id}_i(\bar{\x}_i) = \textstyle\vect^{N_i}_{\alpha = 1}\{ \hh^\mathrm{id}_i(\bar{\x}_i; j_\alpha)\}.
\end{equation}
The final noisy indirect measurement model is given as
\begin{equation}
    \label{eq:dis_indirect_noisy}
    \y^\mathrm{id}_i = \hh^\mathrm{id}_i(\bar{\x}_i) + \bm{\nu}_a
\end{equation}
where $\bm{\nu}_a = \textstyle\diag^{p_{\mathrm{id}}}_{\beta=1}\{\nu_\beta + \nu_{d,\beta}\}$ with $p_{\mathrm{id}} = \sum^{N_i}_{\alpha=1}|\mathcal{N}_{i} \cap \mathcal{N}_{j_\alpha}|$.

Moreover, we assume that all velocity inputs are imperfect due to actuator noise $\Delta \uu_i$ for agent $i$, with which we also define $\Delta \uu_{ij_\alpha} = \vect\{\Delta \uu_i, \Delta \uu_{j_\alpha}\}$ and $\Delta \bar{\uu}_i = \vect\{\Delta \uu_i, \textstyle\vect^{N_i}_{\alpha=1} \{\Delta \uu_{j_\alpha}\} \}$. Referring to \eqref{eq:dy_aug}, \eqref{eq:dis_direct_noisy} and \eqref{eq:dis_indirect_noisy}, the full-CRL (fCRL) model with the augmented dynamics and both direct and indirect measurements is given as
\begin{equation}
\label{eq:fcrl}
    \text{fCRL}:\left \{
    \begin{aligned}
    \dot{\bar{\x}}_i &= \bar{\g}_i(\bar{\x}_i)(\bar{\uu}_i + \Delta\bar{\uu}_i) \\
    \begin{bmatrix}
        \y^\mathrm{d}_i \\
        \y^\mathrm{id}_i
    \end{bmatrix}
    &=
    \begin{bmatrix}
        \hh^\mathrm{d}_i(\bar{\x}_i) \\
        \hh^\mathrm{id}_i(\bar{\x}_i)
    \end{bmatrix}
    +
    \begin{bmatrix}
        \bm{\nu} \\
        \bm{\nu}_a
    \end{bmatrix}
    \end{aligned}
    \right. .
\end{equation}

For comparative study, we also introduce the following two models: i) the half-CRL (hCRL) model with the augmented dynamics and only direct measurements, ii) the non-CRL (nCRL) model which is simply \textit{a collection} of the peer-to-peer dynamics in \eqref{eq:dy_pair} for agent pairs $(i,j_\alpha)$ without state and input augmentation, \sven{$\forall j_\alpha \in \mathcal{N}_i$}. The details are given below:
% hCRL modeling
\begin{equation}
\label{eq:hcrl}
    \hspace{-3.3cm}
    \text{hCRL}:\left \{
    \begin{aligned}
    \dot{\bar{\x}}_i &= \bar{\g}_i(\bar{\x}_i)(\bar{\uu}_i + \Delta\bar{\uu}_i) \\
        \y^\mathrm{d}_i
    &=
        \hh^\mathrm{d}_i(\bar{\x}_i)
    +
        \bm{\nu} 
    \end{aligned}
    \right. ,
\end{equation}
% nCRL modeling
\begin{equation}
\label{eq:ncrl}
    %\hspace{0cm}
    \text{nCRL}:\bigg\{ \left \{
    \begin{aligned}
    \dot{\x}_{ij_\alpha} &= \g(\x_{ij_\alpha})(\uu_{ij_\alpha} + \Delta \uu_{ij_\alpha})\\
    y_{ij_\alpha} &= \|\p_{ij_\alpha}\| + \nu_\alpha
    \end{aligned}
    \right. \bigg\}_{\{j_\alpha \in \mathcal{N}_i\}}.
\end{equation}
\begin{remark}
    The 3 dynamic models (i.e., fCRL, hCRL, and nCRL) are all continuous-time nonlinear control systems. In addition, they are all \textit{drift-free} and \textit{input-affine}, which perfectly fits the general system description in \eqref{eq:sys_math}.
\end{remark}

==> content_file/3.2-Differential_Geometry.tex <==
\subsection{Knowledge from Differential Geometry}
Consider a drift-free input-affine nonlinear control system
\begin{equation}
\label{eq:sys_math}
\left \{
\begin{aligned}
    \dot{\x} &= \sum\nolimits^{m}_{i=1}\g_{i}(\x,t)u_i \\
    \y &= [h_1(\x), h_2(\x), \cdots, h_p(\x)]^\top
\end{aligned}
\right. ,
\end{equation}
where $\x$ evolves in a $\mathcal{C}^\infty-\text{manifold}$ $\mathcal{M}$ of dimension $n$, $\g_{i}(\x,t)$ are time-varying (TV) vector fields in $\mathcal{M}$, and $h_i(\x)$ are time-invariant (TI) scalar fields also defined on $\mathcal{M}$. Besides, all functions are $\mathcal{C}^\infty$ functions of their arguments. The time $t$ belongs to an open interval $\mathcal{I}\subseteq \mathbb{R}$, and we denote $\uM = \mathcal{I}\times \mathcal{M}$. To analyze the above system, we present some basic differential geometric tools.
\begin{definition}[Lie Derivative]
Given a scalar function $h(\x):\mathcal{M} \mapsto \mathbb{R}$, and a vector field $\g(\x,t): \uM \mapsto \mathcal{M}$. The \textit{Lie derivative} of a covector $\mathrm{d}h$ with respect to $\x$ is defined as
\begin{equation}
    \label{eq:lie_derivative}
    \cL_{\g}\mathrm{d}h = \mathrm{d}(\cL_{\g}h) = \mathrm{d}(\langle \frac{\partial h}{\partial \x}, \g(\x,t)\rangle),
\end{equation}
where $\mathrm{d}h$, being the dual of $\g(\x,t)$, is a special type of covector called \textit{exact differential}, \sven{and $\langle \cdot,\cdot\rangle$ denotes the inner product of two vector fields}. Further, a set of \textit{covectors} $\mathrm{d} h_i$ can form a \textit{codistribution} $\Xi = \text{span}\{\mathrm{d} h_i\}$\cite{isidori1985nonlinear}, and the Lie derivative of the codistribution is $\cL_{\g}\Xi = \text{span}\{\cL_{\g}\xi | \forall \xi \in \Xi\}$. 
%In addition, the Lie derivative can be recursively defined as
%\begin{equation}
%\label{eq:lie_recursion}
    %\cL^r_{\g}\mathrm{d}h = \mathrm{d}(\cL^r_{\g}h) = \mathrm{d}(\langle \cL^{r-1}_{\g}\mathrm{d}h, \g \rangle) \;(r \geq 1), 
%\end{equation}
\end{definition}
%with the special case being $\cL^0_{\g}\mathrm{d}h := \mathrm{d}h$.

To analyze the time-varying system in \eqref{eq:sys_math}, we introduce the \textit{augmented Lie derivative} \cite{martinelli2022extension} for a covector $\mathrm{d}h$ as
\begin{equation}
    \label{eq:lie_newoperator}
    \dot{\cL}_{\g}\mathrm{d}h = \cL_{\g}\mathrm{d}h + \frac{\partial \mathrm{d}h}{\partial t}.
\end{equation}
Besides, this new derivative permits a recursive operation as
\begin{equation}
    \dot{\cL}^r_{\g}\mathrm{d}h = \dot{\cL}_{\g}(\dot{\cL}^{r-1}_{\g}\mathrm{d}h),  \quad (r \in \mathbb{Z}_+),
\end{equation}
with the initial case being $\dot{\cL}^0_{\g}\mathrm{d}h := \mathrm{d}h$. Likewise, the augmented Lie derivative can also act upon codistributions. The above geometric tools will be used for the following \textit{observability} analysis.


==> content_file/3.3-Observability.tex <==
\subsection{Observability Analysis}
For the basic peer-to-peer \chang{localization model}, we only have a single distance as measurement, from which we need to decide whether our interested state (i.e., $\p_{ij}$) can be reconstructed. Therefore, we need to analyze the observability of the system. Noting the dynamics of the relative heading $\psi_{ij}$ is decoupled from that of the position $\p_{ij}$ (cf. \ref{eq:dy_aug_compact}), \chang{we thus only consider the position dynamics given that $\psi_{ij}$ is also not our interested state.} After decoupling $\psi_{ij}$, the position dynamics should be treated as a TV \sven{nonlinear system} with $\psi_{ij}(t)$ being the varying parameter. \chang{The resulting peer-to-peer relative dynamics and augmented dynamics are given in \eqref{eq:sub_position_dynamics} and \eqref{eq:sub_position_augdynamics}, respectively.
\begin{equation}
    \label{eq:sub_position_dynamics}
    \left\{
    \begin{aligned}
        \p_{ij} &= \g(\p_{ij}, \uu_{ij}, t) = \bR(\psi_{ij}(t))\vv_j - \vv_i - S\dot{\psi}_i \p_{ij} \\
        y &= h(\p_{ij}) = \|\p_{ij}\|
    \end{aligned}
    \right. ,
\end{equation}
\begin{equation}
    \label{eq:sub_position_augdynamics}
    \left\{
    \begin{aligned}
        \bar{\p}_{i} &= \bar{\g}(\bar{\p}_{i}, \bar{\uu}_{i}, t) \\
            \y^\mathrm{d}_i
                &=
            \hh^\mathrm{d}_i(\bar{\p}_i) \\
            \big(\y^\mathrm{id}_i
                &=
            \hh^\mathrm{id}_i(\bar{\p}_i)\big)
    \end{aligned}
    \right. ,
\end{equation}
where in \eqref{eq:sub_position_augdynamics} $\bar{\g}(\bar{\p}_{i}, \bar{\uu}_{i}, t) = \textstyle\vect^{N_i}_{\alpha=1}\{\g(\p_{ij_\alpha}, \uu_{ij_\alpha}, t)\}$, and $\y^\mathrm{d}_i$ and $\y^\mathrm{id}_i$ are constructed similarly as in \eqref{eq:fcrl} (with details given in \eqref{eq:dis_direct}, \eqref{eq:dis_indirect_neighborwise} and \eqref{eq:dis_indirect_all}). We start with analyzing the peer-to-peer system given in \eqref{eq:sub_position_dynamics}. The observability analysis requires checking the rank of the following observability matrix.}
\begin{equation}
    \label{eq:observability_matrix}
    \OB = 
    \begin{bmatrix}
        \dot{\cL}^0_{\g}\mathrm{d}h \\
        \dot{\cL}^1_{\g}\mathrm{d}h \\
        \dot{\cL}^2_{\g}\mathrm{d}h
    \end{bmatrix}.
\end{equation}
If $\OB$ is of \textit{full rank}, then the TV system is \textit{weakly locally observable} \cite{martinelli2022extension}, otherwise, the system is \textit{unobservable}.

In the following calculation, only the coefficients of the basis $(\{\mathrm{d}x_{ij}, \mathrm{d}y_{ij}, \mathrm{d}z_{ij}\})$ are kept, whereas the basis itself is omitted for simplicity. In addition, all coefficients are multiplied by the non-zero term $2\|\p_{ij}\|$ (i.e., two agents do not collide), which does not affect the rank of $\OB$. After calculation, the augmented Lie derivatives are given as
\begin{subequations}
    \label{eq:explicit_lie_derivative}
    \begin{align}
        \dot{\cL}^0_{\g}\mathrm{d}h &= \p^\top_{ij}, \\
        \dot{\cL}^1_{\g}\mathrm{d}h &= \big[\bR(\psi_{ij}(t))\vv_j - \vv_i\big]^\top,\\
        %\dot{\cL}^2_{\g}\mathrm{d}h &= \dot{\psi}_i\big[\vv_i - \bR(\psi_{ij}(t))\vv_j\big]^\top S + \notag \\
        %&\quad \quad \quad + \dot{\psi}_{ij}(t)\big[\dot{\bR}(\psi_{ij})\vv_j\big]^\top, \\
        %\dot{\cL}^2_{\g}\mathrm{d}h &= \big[\dot{\psi}_j\dot{\bR}(\psi_{ij})\vv_j + \dot{\psi}_i S^\top\vv_i \big]^\top
        \dot{\cL}^2_{\g}\mathrm{d}h &= \dot{\psi}_{ij}\vv^\top_j E-\big[\dot{\psi}_j\bR(\psi_{ij})\vv_j - \dot{\psi}_i \vv_i \big]^\top S
    \end{align}
\end{subequations}
where $E = \vect\{\mathbf{0}_{2\times 3}, \mathbf{b}^3_{3}\}$. Combine the above results and express them in specific form, we obtain the specific analytical form of $\OB$ given as 
\begin{equation}
    \label{eq:ob_explicit}
    \begin{bmatrix}
    \begin{array}{c|c|c}
        x_{ij} & y_{ij} & z_{ij} \\
        \hline
        \makecell*[c]{c(\psi_{ij})v_{x,j}- \\ s(\psi_{ij})v_{y,j} - v_{x,i}} 
        & \makecell*[c]{s(\psi_{ij})v_{x,j}+ \\ c(\psi_{ij})v_{y,j} - v_{y,i}} 
        &   v_{z,j} - v_{z,i} \\
        \hline
        \makecell*[c]{-\dot{\psi}_j s(\psi_{ij})v_{x,j} \\ -\dot{\psi}_j c(\psi_{ij})v_{y,j} \\ + \dot{\psi}_i v_{y,i}} 
        & \makecell*[c]{\dot{\psi}_j c(\psi_{ij})v_{x,j} \\ -\dot{\psi}_j s(\psi_{ij})v_{y,j} \\ - \dot{\psi}_i v_{x,i}} 
        &   v_{z,j} (\dot{\psi}_j - \dot{\psi}_i)
    \end{array}
    \end{bmatrix}.\notag 
\end{equation}
We further denote the relative velocity $\bR(\psi_{ij}(t))\vv_j - \vv_i$ as $\vv_{ij} = [v_{x,ij}, v_{y,ij}, v_{z,ij}]^\top$. Though a complete analysis of the observability is unattainable since the determinant of $\OB$ is difficult to compute, we can still find \textit{unobservable} subspace which has clear physical interpretation:
\begin{enumerate}
    \item Relative velocity is zero (i.e., $\vv_{ij} = \mathbf{0}$, \textbf{parallel motion}): $\OB[2] = \mathbf{0}$.
    \item Relative velocity is \textbf{aligned} with the relative position (i.e., the relative position \textbf{does not change its direction}): $\OB[1] = K\OB[2] (K \neq 0)$.
    \item Two agents move in a \textbf{fixed horizontal plane} ($z_{ij} = v_{z,j} - v_{z,i} = 0$), plus that the localized agent $j$ \textbf{does not have vertical velocity} ($v_{z,j} = 0$) or two agents have the \textbf{same heading rate} ($\dot{\psi}_j - \dot{\psi}_i = 0$): $\OB^\top[3] = \mathbf{0}$.
    \item Two agents have the \textbf{same heading rate} ($\dot{\psi}_j - \dot{\psi}_i = 0$) have \textbf{no relative altitude} ($z_{ij} = 0$), plus the condition $x_{ij}v_{x,ij} + y_{ij}v_{y,ij} = 0$: $\OB[1] = K\OB[3] (K \neq 0)$
    %\item Two agents have the \textbf{same heading rate} ($\dot{\psi}_j - \dot{\psi}_i = 0$) and do have have relative displacement along y-axis of $\mathcal{F}^i_{H}$ ($y_{ij} = 0$), plus that the relative velocity satisfies $$
    \item Relative \textit{scaled} velocity (scaled by heading rate) is zero ($\dot{\psi}_j\bR(\psi_{ij})\vv_j - \dot{\psi}_i \vv_i = 0$), plus that the localized agent $j$ \textbf{does not have vertical velocity} ($v_{z,j} = 0$): $\OB[3] = \mathbf{0}$.
\end{enumerate}

The above observability analysis directly suits the nCRL model due to its dynamics being fully decoupled for each agent pair $(i,j_\alpha), j_\alpha \in \mathcal{N}_i$. 

Regarding the hCRL model, though $\uu_i$ perturbs the dynamics of each agent pair in an integrated manner, both the dynamics $\g^c(\p_{ij_\alpha}, \uu_{ij_\alpha}, t)$ and the measurement model $h_{ij_\alpha} = \|\p_{ij_\alpha}\|$ are decoupled in terms of the state $\x_{ij} (\p_{ij})$. Correspondingly, if we denote the observability matrix for agent pair $(i,j_\alpha)$ using the direct measurement $h(\p_{ij_\alpha})$ as $\OB^{\text{d}}(i,j_\alpha)$, the resulting observability matrix for the hCRL has a \textit{diagonal} structure as $\OB_{\text{hCRL}} = \textstyle\diag^{N_i}_{\alpha=1}\{\OB^{\text{d}}(i,j_\alpha)\}$, from which we can easily conclude that the observability for the hCRL model can be analyzed in a \textit{pair-wise} manner same as that for the nCRL model. 

For fCRL model where indirect measurements are also present, the observable subspace can be expanded. Particularly, if the number of indirect measurements $p_{\text{id}} \geq 2N_i$ (i.e., each neighbor provides at least $2$ indirect measurements on average), the total number of measurements (i.e., counting both direct and indirect ones) will be greater than the number of interested states $3N_i$, then the fCRL system is \textit{fully} observable even without the excitation of control. In general cases where $p_{\text{id}} < 2N_i$, more detailed investigation is required, and we start with the simplest case where we deal with the 3 agent tuple $(i, j_1, j_2)$ without loss of generality. The partial observability matrix for output $h_\beta$ will be denoted as $\OB(h_\beta)$, $(\beta = 1,2,3)$. For direct measurements $h_1 = \|\p_{ij_1}\|$ and $h_2 = \|\p_{ij_2}\|$, we can first easily obtain $\OB(h_1)$ and $\OB(h_2)$ as
\begin{subequations}
    \label{eq:partial_independent_j1j2}
    \begin{align}
        \label{eq:partial_j1}
        \OB(h_1) &= [\OB^{\text{d}}(i,j_1), \mathbf{0}_{3 \times 3}]/\|\p_{ij_1}\|, \\
        \label{eq:partial_j2}
        \OB(h_2) &= [\mathbf{0}_{3 \times 3}, \OB^{\text{d}}(i,j_2)]/\|\p_{ij_2}\|,
    \end{align}
\end{subequations}
For $h_3 = \|\p_{ij_1} - \p_{ij_2}\|$, after computation, we have
\begin{equation}
    \label{eq:partial_j1j2}
    \OB(h_3) = [\OB^{\text{id}}(j_1,j_2), \OB^{\text{id}}(j_2,j_1)],
\end{equation}
where $\OB^{\text{id}}(j_1,j_2)$ is given as
\begin{equation}
    \label{eq:ob_indirect_detail}
    \OB^{\text{id}}(j_1,j_2) = 
    \begin{bmatrix}[2.5]
    \begin{array}{c}
        \p^\top_{ij_1} - \p^\top_{ij_2} \\
        \hline
        [R(\psi_{ij_1})\vv_{j_1} - R(\psi_{ij_1})\vv_{j_2}]^\top \\
        \hline
        \makecell[c]{
        (\dot{\psi}_{ij_1}\vv_{j_1} - \dot{\psi}_{ij_2}\vv_{j_2})^\top E
        \\
        -[\dot{\psi}_{ij_1}R(\psi_{ij_1})\vv_{j_1} - \dot{\psi}_{ij_2}R(\psi_{ij_2})\vv_{j_2}]^\top S
        }
    \end{array}
    \end{bmatrix},\notag
\end{equation}
where all entries in $\OB^{\text{id}}(j_1,j_2)$ are multiplied by the same factor $\|\p_{ij_1} - \p_{ij_2}\|$. Besides, it can be easily verified that $\OB^{\text{id}}(j_1,j_2) + \OB^{\text{id}}(j_2,j_1) = 0$, with which \eqref{eq:partial_j1j2} can be written as
\begin{equation}
    \label{eq:parital_j1j2_modified}
    \OB(h_3) = [\OB^{\text{id}}(j_1,j_2), -\OB^{\text{id}}(j_1,j_2)].
\end{equation}
The final observability matrix is thus given as
\begin{equation}
    \label{eq:ob_3agentfinal}
    \OB(i,j_1,j_2) = 
    \begin{bmatrix}[2]
        \frac{\OB^{\text{d}}(i,j_1)}{\|\p_{ij_1}\|} & \mathbf{0}_{3 \times 3} \\
        \mathbf{0}_{3 \times 3} & \frac{\OB^{\text{d}}(i,j_2)}{\|\p_{ij_2}\|} \\
        \frac{\OB^{\text{id}}(j_1,j_2)}{\|\p_{ij_1} - \p_{ij_2}\|} & -\frac{\OB^{\text{id}}(j_1,j_2)}{\|\p_{ij_1} - \p_{ij_2}\|}
    \end{bmatrix}
\end{equation}
\chang{We then discuss how the observable subspace can be expanded by imposing extra stringent conditions on the previously identified unobservable subspace. In the following analysis, we only discuss the cases where the previously identified $5$ unobservable conditions hold independently, whereas the cases in which multiple conditions are satisfied simultaneously will not be further investigated.} 
\begin{enumerate}
    \item Parallel motion
    \begin{itemize}
        \item \chang{If either $(i,j_1)$ or $(i,j_2)$ is in parallel motion, then the system is always observable in that $\OB^{\text{id}}(j_1,j_2)[1] \neq 0$ always holds true.}
        \item \chang{If both $(i,j_1)$ and $(i,j_2)$ are in parallel motion (i.e., all 3 agents are in parallel motion), then the system is still observable if the relative scaled velocity of pair $(j_1, j_2)$ is non-zero (i.e., $\OB^{\text{id}}(j_1,j_2)[3] \neq 0$)}
    \end{itemize}
    \item Relative velocity aligned with the relative position
    \begin{itemize}
        \item \chang{If either $(i,j_1)$ or $(i,j_2)$ falls in this aligning condition, then the system is always observable in that $\OB^{\text{id}}(j_1,j_2)[1] \neq 0$ always holds true.}
        \item \chang{If both pair $(i,j_1)$ and $(i,j_2)$ satisfy this aligning condition, then the system is still observable if pair $(j_1, j_2)$ does not meet this condition. Further, even if $(j_1, j_2)$ also satisfies this aligning condition, then the system is still observable if the relative scaled velocity of pair $(j_1, j_2)$ is non-zero (i.e., $\OB^{\text{id}}(j_1,j_2)[3] \neq 0$).} 
    \end{itemize}
    \item Fixed horizontal plane plus zero vertical velocity \\
    \chang{If at least one of the two pairs $(i, j_1)$ and $(i, j_2)$ satisfies the condition that $i$ and $j_1$ ($j_2$) moves in the same horizontal plane and $j_1$ ($j_2$) does not have vertical velocity, then the system is still observable if any one of the below conditions holds: i) $j_1$ and $j_2$ have altitude difference 2) $j_1$ and $j_2$ have different vertical velocity 3) the relative scaled vertical velocity of pair $(j_1, j_2)$ is non-zero.}
\end{enumerate}
\chang{The remaining identified conditions 4) and 5) in the previous peer-to-peer observability analysis are unlikely to satisfy in general. Considering that $3$ extra rows are added to the observability matrix due to the additional indirect measurement, the unobservable subspace corresponding to conditions 4) and 5) is diminished to a large extent.}

\chang{For the general fCRL model of agent $i$ and its neighbor set $\mathcal{N}_i$, its observability matrix $\OB(i,\mathcal{N}_i)$ is given as}
\chang{
\begin{equation}
\def\arraystretch{2}
    \label{eq:ob_fcrl_general}
    \begin{bNiceMatrix}[first-row, last-col, respect-arraystretch]
        \mathrm{d}\p_{ij_1} & \mathrm{d}\p_{ij_2} & \cdots & \mathrm{d}\p_{ij_{N_i}} & \\
        \frac{\OB^{\text{d}}(i,j_1)}{\|\p_{ij_1}\|} & \mathbf{0}_{3 \times 3} & \cdots & \mathbf{0}_{3 \times 3} & d_{ij_1}\\
        \mathbf{0}_{3 \times 3} & \frac{\OB^{\text{d}}(i,j_2)}{\|\p_{ij_2}\|} & \cdots & \mathbf{0}_{3 \times 3} & d_{ij_2}\\
        \vdots & & \ddots & \vdots & \vdots \\
        \mathbf{0}_{3 \times 3} & \cdots & & \frac{\OB^{\text{d}}(i,j_{N_i})}{\|\p_{ij_{N_i}}\|} & d_{ij_{N_i}} \\
        \hline
        \frac{\OB^{\text{id}}(j_1,j_2)}{\|\p_{ij_1} - \p_{ij_2}\|} & -\frac{\OB^{\text{id}}(j_1,j_2)}{\|\p_{ij_1} - \p_{ij_2}\|} & \cdots & \mathbf{0}_{3 \times 3} & d_{j_1j_2}\\
        \frac{\OB^{\text{id}}(j_1,j_{N_i})}{\|\p_{ij_1} - \p_{ij_{N_i}}\|} & \mathbf{0}_{3 \times 3} & \cdots & -\frac{\OB^{\text{id}}(j_1,j_{N_i})}{\|\p_{ij_1} - \p_{ij_{N_i}}\|} & d_{j_1j_{N_i}} \\
        \vdots & \vdots & \vdots & \vdots & \vdots
    \end{bNiceMatrix}, \notag
\end{equation}
where the upper diagonal matrix is fixed and the lower part depends on the type of indirect measurements. Specifically, the direct measurement $d_{ij_\alpha}$ and the indirect measurement $d_{j_\alpha j_\beta}$ contribute, respectively, to the following two blocks:
\begin{equation}
    \label{eq:ob_indi_detial}
    \left \{
    \begin{aligned}
        d_{ij_\alpha}: \;& \mathbf{b}^{N_i}_{\alpha} \otimes \frac{\OB^{\text{id}}(j_i,j_{\alpha})}{\|\p_{ij_\alpha}\|} \\
        d_{j_\alpha j_\beta}: \;& (\mathbf{b}^{N_i}_{\alpha} - \mathbf{b}^{N_i}_{\beta}) \otimes \frac{\OB^{\text{id}}(j_\alpha,j_{\beta})}{\|\p_{ij_\alpha} - \p_{ij_{\beta}}\|}
    \end{aligned}
    \right. .
\end{equation}
Based on the special structure of the observability matrix, the general rule of thumb is that the more indirect measurements that agent $j_\alpha$ is coupled, the more the unobservable subspace corresponding to the state $\p_{ij_\alpha}$ diminishes.
}










